On the deformation theory of Fourier-Mukai transforms between Calabi-Yau varieties

We study the deformation theory of fully faithful Fourier-Mukai transforms in both characteristic zero and mixed characteristic. Our main result shows that obstructions to deforming such transforms can be completely controlled by Hodge theory when the source variety has trivial canonical bundle, generalizing work of Addington-Thomas and Lieblich-Olsson. The main technical contribution is a formula for the obstruction class measuring the failure of a Chern character to remain within the Hodge filtration as a cup product with a (derived) Kodaira-Spencer class.

==> improving_quillen.tex <==
%!TEX root = main.tex
In \cite{quillen-rings}, Quillen introduced the notion of a quasi-regular ideal. We warn the reader that is not equivalent to the definition in \stacksref{07CU}.
\begin{definition}
Let $A$ be a ring. We say an ideal $I \subseteq A$ is quasi-regular if
\begin{enumerate}
\item $I / I^2$ is a flat $A / I$-module.
\item The canonical map $\wedge_q(I / I^2) \to \Tor_q^A(A / I, A / I)$ constructed in \cite[Definition 8.4]{quillen-rings} is an isomorphism for all $q \geq 0$. 
\end{enumerate}
\begin{definition}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. We say that $I$ is \emph{quasi-regular} if $I_n \subseteq A_n$ is a quasi-regular ideal for all $n$. 
\end{definition}
Then Quillen proved the following (see \cite[Theorem 8.8]{quillen-rings}).
\begin{theorem}[Quillen's convergence theorem]
Let $A$ be a simplicial ring, and $I \subseteq A$ be a simplicial ideal. If $I$ is quasi-regular and $\pi_0(I) = 0$, then $A$ is $I$-adically complete, i.e. the natural map $A \to \derR\lim (A / I^n)$ is a weak equivalence of simplicial rings.
\end{theorem}
The goal of this chapter is to show the assumption $\pi_0(I) = 0$ in the theorem above can be weakened to merely assuming the image of $\pi_0(I)$ in $\pi_0(A)$ is a nilpotent ideal. 
\begin{theorem}[Quillen's convergence theorem, improved version]\label{thm_quillen_convergence_thm_improved}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a quasi-regular simplicial ideal. Suppose the image of $\pi_0(I)$ in $\pi_0(A)$ is nilpotent. Then $A$ is $I$-adically complete, i.e. the natural map $A \to \derR \lim A / I^n$ is a weak equivalence of simplicial rings.
\end{theorem}
Note that the assumptions of the theorem do not necessarily imply that $\pi_0(I^k) = 0$ for some $k > 0$, in fact it could happen that $\pi_0(I^k)$ is always nontrivial.
\end{definition}

\section{Strict-essentially-zero systems}
Before we can prove Theorem \ref{thm_quillen_convergence_thm_improved}, we need an intermezzo on strict-essentially-zero systems (or Artin-Rees-zero systems, see \cite[expos\'e V, 2.2]{sga5}), which will be our main computational tool. Let $\mathcal{A}$ be an abelian category. Write $\mathcal{C} = \Fun(\NN^\op, \mathcal{A})$ for the category of inverse systems in $\mathcal{A}$. 
\begin{definition}
A system $\{K_n\}_n \in \mathcal{C}$ is \emph{strict-essentially-zero} if there exists an integer $k > 0$ such that all maps $K_n \to K_m$ are zero for $n - m \geq k$. 
\end{definition}
We write $\mathcal{C}_0$ for the full subcategory of $\mathcal{C}$ of strict-essentially-zero systems.

The key motivation for studying strict-essentially-zero systems is the following.
\begin{lemma}\label{lem_sez_rlim}
Suppose $\{K_n\}_n \in \mathcal{C}_0$. Then $\lim K_n = \derR^1 \lim K_n = 0$.
\end{lemma}
\begin{proof}
The fact that $\lim K_n = 0$ follows directly from the definition of the direct limit. The condition that $\{K_n\}_n$ is strict-essentially-zero also implies that $\{K_n\}_n$ satisfies the Mittag-Leffler condition, hence $\derR^1 \lim K_n = 0$. 
\end{proof}
The following lemma is key in studying strict-essentially-zero systems. It implies that $\mathcal{C}_0$ is a Serre subcategory, see \stacksref{02MN}.
\begin{lemma}\label{lemma_strict-essentially-zero-triangle}
Suppose we are given a diagram 
\[
A_n \xrightarrow{f_n} B_n \xrightarrow{g_n} C_n
\]
in $\Fun(\NN^\op, \mathcal{A})$ such that  $\ker(g_n) \subseteq \im(f_n)$ for all $n$. If $\{A_n\}_n$ and $\{C_n\}_n$ are strict-essentially-zero, then so is $\{B_n\}_n$.
\end{lemma}
\begin{proof}
Let $k$ such that $A_n \to A_m$ is the zero map for $n - m \geq k$, and $k'$ such that $C_n \to C_m$ is zero for $n - m \geq k'$.

We claim that $B_n \to B_m$ is zero for $n - m \geq k + k'$. Indeed, let $n, m \in \NN$ such that $n - m \geq k + k'$. Write $\ell = n - k'$, so that $n - \ell = k'$ and $\ell - m \geq k$. Consider the diagram
\[
\begin{tikzcd}
A_n \rar \dar & B_n \dar \rar& C_n \dar \\
A_\ell \rar  \dar& B_\ell \rar \dar& C_\ell  \dar\\
A_m \rar & B_m \rar& C_m
\end{tikzcd}
\]
Since $n - \ell = k'$ the map $C_n \to C_\ell$ is the zero map, so we may conclude that $\im(B_n \to B_\ell) \subseteq \im(A_\ell \to B_\ell)$. But $\ell - m \geq k$, hence $A_\ell \to A_m$ is the zero map, therefore $\im(A_\ell \to B_\ell)$ maps to $0$ in $B_m$. It follows that $B_n \to B_m$ is the zero map.
\end{proof}

\begin{corollary}
The category $\mathcal{C}_0$ is a Serre subcategory of $\mathcal{C}$. There exists an abelian category $\cmod$ and an exact functor
\[
F \colon \mathcal{C} \to \cmod
\]
which is essentially surjective and has kernel $\mathcal{C}_0$. 
\end{corollary}
\begin{proof}
See \stacksref{02MS}.
\end{proof}
To end this section, we develop some machinery to detect when an element of $\mathcal{C}$ actually lies in $\mathcal{C}_0$. 
\begin{definition}
For $\{A_n\}_n \in \mathcal{C}$ and $c > 0$, we define the \emph{shift map} as the map $\{A_{n + c}\}_n \to \{A_n\}_n$ in $\mathcal{C}$ given by the map $A_{n + c} \to A_n$ in each degree.
\end{definition}
\begin{definition}
Let $f \colon A \to B$ be a morphism in $\mathcal{C}$. Then $f$ is said to be \emph{strict-essentially-zero} if $F(f) = 0$. 
\end{definition}
\begin{lemma}
For any $\{A_n\}_n \in \mathcal{C}$ and $c > 0$, the shift map $\{A_{n + c}\}_n \to \{A_n\}_n$ maps to an isomorphism in $\mathcal{C} / \mathcal{C}_0$. 
\end{lemma}
\begin{proof}
This follows since $\{\ker(A_{n + c} \to A_n)\}_n$ and $\{\mathrm{coker}(A_{n + c} \to A_n)\}_n$ lie in $\mathcal{C}_0$. 
\end{proof}
\begin{corollary}\label{corol_shift_sez}
Let $\{A_n\}_n \in \mathcal{C}$ and $c > 0$. If the shift map $\{A_{n + c}\}_n \to \{A_n\}_n$ is strict-essentially-zero, then $\{A_n\}_n \in \mathcal{C}_0$. 
\end{corollary}
\section{Improving Quillen's result}
We now move on to proving Theorem \ref{thm_quillen_convergence_thm_improved}. The basic strategy is to prove that $\{\pi_k(I^n)\}_n$ is strict-essentially-zero by induction on $k$. We highly recommend the reader to compare with the proof of \cite[Theorem 8.8]{quillen-rings}, in which it is shown that $\pi_k(I^{k + 1}) = 0$ by induction on $k$ after assuming $\pi_0(I) = 0$.

Write $\mathcal{C} = \Fun(\NN^\op, \Ab)$ and let $\mathcal{C}_0$ be the full subcategory of strict-essentially-zero systems. By Lemma \ref{lemma_strict-essentially-zero-triangle}, $\mathcal{C}_0$ is a Serre subcategory of $\mathcal{C}$. 

By Corollary \ref{corol_shift_sez}, to show that $\{\pi_k(I^n)\}_n \in \mathcal{C}_0$, it suffices to show that the shift map 
\[
\{\pi_k(I^{n + c}) \}_n\to \{\pi_k(I^n)\}_n
\]
is strict-essentially-zero, which motivates what follows.

The following is a slight improvement of \cite[Proposition 8.5]{quillen-rings}, and is the basis for Theorem \ref{thm_quillen_convergence_thm_improved}. 
\begin{lemma} \label{lemma_discete_tor_sez}
Let $A$ be a ring and let $I \subseteq A$ be a quasi-regular ideal. For fixed $q > 0$ and $k > 0$, the system $\{\Tor^A_q(A / I^k, A  /I^n)\}_n \in \mathcal{C}_0$.
\end{lemma}
\begin{proof}
We give a proof by induction on $k$ for fixed $q > 0$. The case $k = 1$ is proven in \cite[Proposition 8.5, $\text{B}_q$]{quillen-rings}, in fact Quillen shows that 
\[
\Tor_q(A / I, A / I^n) \to \Tor_q(A / I, A / I^{n - 1})
\]
is the zero map for all $q$ and $n$. 

Now suppose the statement holds for $k - 1$, we show it holds for $k$. Note that by \cite[Proposition 8.5, $\text{A}_k$]{quillen-rings} the $A / I$-module $I^{k - 1 }/ I^k$ is flat, hence 
\begin{align*}
\Tor_q^{A}(I^{k - 1} / I^k, A / I^n) &\cong \coh_q\(I^{k - 1} / I^k \otimes^{\derL}_A A / I^n\) \\
&\cong \coh_q\(I^{k - 1} / I^k \otimes^{\derL}_{A / I} \(A / I \otimes^{\derL}_A A / I^n\)\) \\
&\cong I^{k - 1} / I^k \otimes_{A / I} \coh_q\( A / I \otimes^{\derL}_A A / I^n\) \\
&\cong I^{k - 1} / I^k \otimes_{A / I} \Tor_q^A\( A / I, A / I^n\)
\end{align*}
is strict-essentially-zero (as an inverse system in $n$). The short exact sequence
\[
0 \to I^{k - 1} / I^k \to A / I^k \to A  / I^{k - 1} \to 0
\]
induces an exact sequence
\[
\Tor_q(I^{k - 1} / I^k, A / I^n) \to \Tor_q(A / I^k, A / I^n) \to \Tor_q(A / I^{k - 1}, A / I^n)
\]
The result now follows from Lemma \ref{lemma_strict-essentially-zero-triangle}, as the rightmost term is strict-essentially-zero by our induction hypotheses, and we already showed the leftmost term was strict-essentially-zero.
\end{proof}

\begin{lemma}\label{lem_pik_basic}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. Suppose the image of $\pi_0(I)$ in $\pi_0(A)$ is  a nilpotent ideal. Then $\{\pi_0(I^n)\}_n \in \mathcal{C}_0$. 
\end{lemma}
\begin{proof}
Let $J$ be the image of $\pi_0(I)$ in $\pi_0(A)$, and let $k > 0$ be such that $J^k = 0$. Note that for any $n$, the image of $\pi_0(I^n)$ in $\pi_0(A)$ is equal to $J^n$. In particular, it follows that $\pi_0(I^k) \to \pi_0(A)$ is the zero map.

Since 
\[
I_0^k \otimes_{A_0} I_0^n \to I_0^{n + k}
\]
is surjective for all $n$, the map $\pi_0(I^k) \otimes_{\pi_0(A)} \pi_0(I^n) \to \pi_0(I^n)$ is surjective for all $n$. Now consider the commutative diagram
\[
\begin{tikzcd}
\dar \pi_0(I^k) \otimes_{\pi_0(A)} \pi_0(I^{n}) \arrow[twoheadrightarrow]{r} & \pi_0(I^{n + k}) \dar \\
\pi_0(A) \otimes_{\pi_0(A)} \pi_0(I^{n}) \arrow[twoheadrightarrow]{r} & \pi_0(I^{n})
\end{tikzcd}
\]
Since the left vertical map is the zero map by assumption, and the top vertical map is surjective, the right vertical map is the zero map as well. We conclude that $\pi_0(I^{n + k}) \to \pi_0(I^n)$ is the zero map for all $n \geq 0$, which proves the lemma. 
\end{proof}

Note that for any simplicial ring $A$, we can consider the graded ring $\pi_*(A)$. Then $\pi_*(I^n)$ is a graded module over this ring for all $n$, and in particular we get graded groups
\[
\Tor_p^{\pi_*(A)}\(\pi_*(I^c), \pi_*(I^n)\)
\]
for all $p, n, c \in \ZZ_{\geq 0}$. We will denote the $\ell$-th graded piece by 
\[
\Tor_p^{\pi_*(A)}\(\pi_*(I^c), \pi_*(I^n)\)_\ell
\]
The following lemma is needed to analyze the spectral sequence from \cite[II, \S 6, Theorem 6]{quillen-ha}. 
\begin{lemma}\label{lemma_graded_tor_sez}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. Let $k > 0$. Suppose that $\{\pi_j(I^n)\}_n \in \mathcal{C}_0$ for all $0 \leq j < k$. Then
\[
\left\{\Tor_p^{\pi_*(A)}\(\pi_*(I^c), \pi_*(I^n)\)_{k - p}\right\}_n \in \mathcal{C}_0
\]
for all $p > 0$ and $c \geq 0$. 
\end{lemma}
\begin{proof}
Let $P_{*, \bullet} \to \pi_*(I^c)$ be a graded projective resolution of $\pi_*(I^c)$ as a $\pi_*(A)$-module. Then in each homological degree $i$, we have a surjection 
\[
\left\{\bigoplus_{a = 0}^{k - p} P_{a, i} \otimes_{\pi_0(A)} \pi_{k - p - a}(I^n)\right\}_n \twoheadrightarrow \left\{ \(P_{*,i} \otimes_{\pi_*(A)} \pi_*(I^n)\)_{k - p}\right\}_n
\]
in $\mathcal{C}$. Since the left hand side is an element of $\mathcal{C}_0$, so is the right-hand side. Since this holds for all $i$, it follows that 
\[
\left\{\coh_p \(\(P_{*,\bullet} \otimes_{\pi_*(A)} \pi_*(I^n)\)_{k - p}\)\right\}_n
\]
is an element of $\mathcal{C}_0$, which is what we needed to show.
\end{proof}
\begin{lemma}\label{lemma_sez_derived_tensor_epi}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. Let $k > 0$. Suppose that $\{\pi_i(I^n)\}_n\in \mathcal{C}_0$ for all $0 \leq i < k$. Then for any $c$, the natural map 
\[
\{\(\pi_*(I^c) \otimes_{\pi_*(A)} \pi_*(I^n)\)_k\}_n \to \{\pi_k(I^c \otimes^\derL_A I^n)\}_n
\]
is an epimorphism in $\cmod$.
\end{lemma}
\begin{proof}
By \cite[II, \S 6, Theorem 6]{quillen-ha} we have a spectral sequence
\[
E^2_{p, q} = \{\Tor_p^{\pi_*(A)}\(\pi_*(I^c), \pi_*(I^n)\)_q\}_n \implies \{\pi_{p + q} (I^c \otimes^{\derL}_A I^n) \}_n
\]
in $\mathcal{C}$. By Lemma \ref{lemma_graded_tor_sez} one has $E^2_{p, k - p} \in \mathcal{C}_0$ for $p > 0$, hence $E^\infty_{p, k - p} \in \mathcal{C}_0$ for $p > 0$. It follows that 
\[
E_{0, k}^\infty \to \{\pi_{k}\(I^c \otimes_A^\derL I^n\)\}_n
\]
is an isomorphism in $\cmod$. The result now follows since $E_{0, k}^2 \to E_{0, k}^\infty$ is an epimorphism (already in $\mathcal{C}$).
\end{proof}

\begin{lemma}\label{lemma_sez_derived_tensor}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. Let $k > 0$. Suppose that $\{\pi_i(I^n)\}_n\in \mathcal{C}_0$ for all $0 \leq i < k$. Then there exists $c > 0$ for which the natural map
\[
 \{\pi_k(I^c \otimes^\derL_A I^n)\}_n \to \{\pi_k(I^n) \}_n
\]
is strict-essentially-zero.
\end{lemma}
\begin{proof}
Let $c$ be such that $\pi_0(I^c) \to \pi_0(A)$ is the zero map. By Lemma \ref{lemma_sez_derived_tensor_epi}, it suffices to show the natural map
\[
\{\(\pi_*(I^c) \otimes_{\pi_*(A)} \pi_*(I^n)\)_k\}_n \to \{\pi_k(I^n)\}_n
\]
is strict-essentially-zero. Note that we have a diagram in $\mathcal{C}$
\[
\begin{tikzcd}
\dar\{ \bigoplus_{a = 0}^k {\pi_a(I^c)} \otimes_{\pi_0(A)} \pi_{k - a}(I^n)\}_n \arrow[twoheadrightarrow]{r} & \{\(\pi_*(I^c) \otimes_{\pi_*(A)} \pi_*(I^n)\)_k \}_n\dar \\
\{\bigoplus_{a = 0}^k {\pi_a(A)} \otimes_{\pi_0(A)} \pi_{k - a}(I^n)\}_n \arrow[twoheadrightarrow]{r} & \{\pi_k(I^n)\}_n
\end{tikzcd}
\]
in which the horizontal arrows are surjections. Since the left vertical map is strict-essentially-zero (note $\{\pi_{k - a}(I^n)\}_n \in \mathcal{C}_0$ for $a > 0$), we get a diagram
\[
\begin{tikzcd}
\{\bigoplus_{a = 0}^k {\pi_a(I^c)} \otimes_{\pi_0(A)} \pi_{k - a}(I^n) \}_n\arrow{dr}{0} \arrow[twoheadrightarrow]{r} & \{\(\pi_*(I^c) \otimes_{\pi_*(A)} \pi_*(I^n)\)_k\}_n \dar \\
 & \{\pi_k(I^n)\}_n
\end{tikzcd}
\]
 in $\mathcal{C} / \mathcal{C}_0$. The result follows.
 \end{proof}
 At first glance, the Lemma below might seem identical to the Lemma above, however this is not quite the case as the derived tensor product has been replaced by the underived version, and $I$ is now assumed to be regular. 
\begin{lemma}\label{lem_constant_tor_sez}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. Let $k > 0$. Suppose that $I$ is quasi-regular, and $\{\pi_i(I^n)\}_n \in \mathcal{C}_0$ for all $0 \leq i < k$. Then there exists $c > 0$ such that 
\[
\{\pi_k(I^c \otimes_A I^n)\}_n \to \{\pi_k(I^n)\}_n
\]
is strict-essentially-zero.
\end{lemma}
\begin{proof}
By Lemma \ref{lemma_sez_derived_tensor}, there exists $c > 0$ such that 
\[
\{\pi_k(I^{c} \otimes^\derL_A I^n)\}_n \to \{\pi_k(I^n)\}_n
\]
is strict-essentially-zero. Now by \cite[II, \S 6, Theorem 6]{quillen-ha}, we have a spectral sequence in $\mathcal{C}$
\begin{align*}
E^2_{pq} &= \{\pi_p(\Tor_q(I^c, I^n))\}_n \implies \{\pi_{p + q}(I^c \otimes^\derL_A I^n)\}_n
\end{align*}
Note that for $q > 0$, one has $\Tor_q(I^c, I^n) = \Tor_{q + 2}(A / I^c, A / I^n)$. Hence by Lemma \ref{lemma_discete_tor_sez} one has $E^2_{p, q} \in \mathcal{C}_0$ for all $q > 0$. It therefore follows that the map $\{\pi_k (I^c \otimes^\derL_A  I^n)\}_n \to E^2_{k,0}$ is an isomorphism in $\mathcal{C} / \mathcal{C}_0$. We thus get a diagram in $\mathcal{C} / \mathcal{C}_0$
\[
\begin{tikzcd}
\{\pi_k(I^c \otimes^\derL_A I^n)\}_n \arrow{r}{\sim} \arrow{dr}{0}& \dar \{\pi_k(I^c \otimes_A I^n)\}_n \\
& \pi_k(I^n)
\end{tikzcd}
\]
The result follows.
\end{proof}
\begin{prop}\label{lem_pik_inductive}
Let $A$ be a simplicial ring, and let $I \subseteq A$ be a simplicial ideal. Let $k > 0$. Suppose that $I$ is quasi-regular, and $\{\pi_0(I^n)\}_n \in \mathcal{C}_0$. Then $\{\pi_k(I^n)\}_n \in \mathcal{C}_0 $ for all $k$. 
\end{prop}
\begin{proof}
By induction on $k$, assume the statement holds for $k' < k$. By Lemma \ref{lem_constant_tor_sez}, there exists $c > 0$ such that $\{\pi_k(I^c \otimes_A I^n)\} \to \{\pi_k(I^n)\}_n$ is strict-essentially-zero. Consider the short exact sequence
\[
\begin{tikzcd}
0 \rar & \Tor_1^A(A / I^c, I^n) \rar&  I^c \otimes_A I^n \rar&  I^{n + c} \rar&0 
\end{tikzcd}
\]
of simplicial $A$-modules, inducing an exact sequence
\[
\begin{tikzcd}
\pi_k(I^c \otimes_A I^n) \rar & \pi_k(I^{n + c}) \rar & \pi_{k - 1}\(\Tor_1^A(A / I^c, I^n)\)
\end{tikzcd}
\]
functorial in $n$. Note that
\[
\{\pi_{k - 1}\(\Tor_1^A(A / I^c, I^n)\)\}_n = \{\pi_{k - 1}\(\Tor_2^A(A / I^c, A / I^n)\)\}_n \in \mathcal{C}_0
\]
by Lemma \ref{lemma_discete_tor_sez}. We thus get a diagram in $\cmod$ 
\[
\begin{tikzcd}
\{\pi_k(I^c \otimes_A I^n)\}_n \arrow{dr}{0} \arrow[twoheadrightarrow]{r} & \dar \{\pi_k(I^{n + c})\}_n  \\
& \{\pi_k(I^n)\}_n
\end{tikzcd}
\]
It follows that the shift map $\{\pi_k(I^{n + c})\}_n \to \{\pi_k(I^n)\}_n$ is strict-essentially-zero, so that we may conclude $\{\pi_k(I^n)\}_n \in \mathcal{C}_0$ by Corollary \ref{corol_shift_sez}.
\end{proof}
Using the above proposition we now prove the promised theorem. 
\begin{proof}[Proof of Theorem \ref{thm_quillen_convergence_thm_improved}]
By Lemma \ref{lem_pik_basic} and Proposition \ref{lem_pik_inductive}, we see that the system $\{\pi_k(I^n)\}_n$ is strict-essentially-zero for all $k \geq 0$. From the short exact sequence of simplicial $A$-modules
\begin{equation}
0 \to I^n \to A \to A / I^n \label{eq_ses_ideal_powers} \to 0
\end{equation}
we obtain exact sequences
\[
\pi_k(A) \to \pi_k(A / I^n) \to \pi_{k - 1}(I^n)
\]
functorial in $n$. Since  $\{\pi_{k - 1}(I^n)\}_n$ is strict-essentially-zero, there exists $c$ such that $\pi_{k - 1}(I^n) \to \pi_{k - 1}(I^m)$ is the zero map for $n - m \geq c$. For fixed $m$ and $n \geq m + c$, we have a commutative diagram
\[
\begin{tikzcd}
\dar \pi_k(A) \rar& \dar \pi_k(A / I^n) \rar& \dar{0} \pi_{k - 1}(I^n) \\
\pi_k(A) \rar& \pi_k(A / I^m) \rar& \pi_{k - 1}(I^m)
\end{tikzcd}
\]
It follows that  the image of $\pi_k(A / I^n)$ in $\pi_k(A / I^m)$ is equal to the image of $\pi_k(A)$, and in particular stabilizes. Thus $\{\pi_k(A / I^n)\}$ satisfies the Mittag-Leffler condition, and $\derR^1 \lim \pi_k(A / I^n) = 0$ for all $k \geq 0$. Since $\{\pi_k(I^n)\}_n$ is strict-essentially-zero, by Lemma \ref{lem_sez_rlim} we conclude that $\derR \lim \pi_k(I^n) = 0$ for all $k \geq 0$. The long exact sequence associated to (\ref{eq_ses_ideal_powers}) together with the fact that $\derR \lim$ is an exact functor then shows that the natural map 
\[
\pi_k(A) \xrightarrow{\sim} \derR \lim \pi_k(A / I^n)
\]
is an isomorphism for all $k$. 

Since we already showed that $\derR^1\lim \pi_k(A / I^n) = 0$, we conclude that the natural map 
\[
\pi_k(A) \xrightarrow{\sim} \lim \pi_k(A / I^n) 
\]
is an isomorphism for all $k$. Furthermore, the Milnor exact sequence
\[
0 \to \derR^1 \lim \pi_{k + 1}(A / I^n) \to \pi_k(\derR \lim A / I^n) \to \lim \pi_k(A / I^n) \to 0
\]
 implies that the map  $ \pi_k(\derR \lim A / I^n) \xrightarrow{\sim} \lim \pi_k(A / I^n)$ is an isomorphism for all $k$. It follows that the natural map
\[
\pi_k(A) \xrightarrow{\sim}  \pi_k(\derR \lim A / I^n)
\]
is an isomorphism for all $k$, as desired. 
\end{proof}
\section{Application: A direct proof of nil-invariance for derived de Rham cohomology in characteristic zero}
In \cite{goodwillie1, goodwillie2}, Goodwillie showed that if $k$ is a $\QQ$-algebra and $A \to B$ is a surjective morphism of (simplicial) associative $k$-algebras with a nilpotent kernel, the natural map
\[
\mathrm{HP}^\bullet(A / k) \to \mathrm{HP}^\bullet(B / k)
\]
on periodic Hochschild homology gives a quasi-isomorphism of chain complexes. Using the Hochschild-Kostant-Rosenberg isomorphism, one may transfer this result to derived de Rham cohomology to show that for any surjective morphism $A \to B$ of commutative $k$-algebras with nilpotent kernel, the natural map
\[
\widehat{\dR}_{A / k} \to \widehat{\dR}_{B / k}
\]
is a quasi-isomorphism, see also \cite{pridham}. In this section we give a direct proof of this result, without comparing to periodic Hochschild homology. 

The idea of the proof is to apply the trick from \cite[Proposition 4.16]{bhatt-cddrc} twice to reduce to the case that $\pi_0(k) \to \pi_0(A)$ is an isomorphism (where now $k$ might no longer be discrete). In this case the statement is obvious since both sides of (\ref{eq_goodwillie_dr}) are isomorphic to $k$ by our improved version of Quillen's convergence theorem. 

\begin{theorem}[Nil-invariance of derived de Rham cohomology]\label{theorem_goodwillie_dr}
Let $k$ be a ring such that $\QQ \subseteq k$, and let $A \to B$ be a morphism in $\CAlg^\an_k$ such that $\pi_0(A) \to \pi_0(B)$ is surjective. If $\ker(\pi_0(A) \to \pi_0(B))$ is a nilpotent ideal in $\pi_0(A)$, then the natural map
\begin{equation}
\widehat{\dR}_{A / k} \to \widehat{\dR}_{B / k} \label{eq_goodwillie_dr}
\end{equation}
is an equivalence in $\CAlg_k$. 
\end{theorem}
Note that although the map is a morphism of filtered $\EE_\infty$-algebras, it is not an equivalence of filtered algebras, as the graded pieces need not be isomorphic. 
\begin{proof}[Proof of Theorem \ref{theorem_goodwillie_dr}]
By Lemma \ref{lem_descent_dr} (descent on the base) and commuting limits with limits we see that the natural map
\[
\widehat{\dR}_{Z / X} \to \lim_\Delta \widehat{\dR}_{Z / \Cech(X \to Y)}
\]
is an equivalence for all $(X \to Y \to Z)\in \Fun(\Delta^2, \CAlg_k^\an)$. Applying this to $k \to A \to A$ and $k \to A \to B$, we get a commutative diagram
\[
\begin{tikzcd}
\widehat{\dR}_{A / k}\dar \rar{\sim} & \lim_\Delta \widehat{\dR}_{A / \Cech(k \to A)} \dar \\
\widehat{\dR}_{B / k} \rar{\sim} & \lim_\Delta \widehat{\dR}_{B / \Cech(k \to A)}
\end{tikzcd}
\]
Since $\pi_0(A^{\otimes n}) \to \pi_0(A)$ is surjective, it suffices to show that for any animated ring $F \in \CAlg_k^\an$ and any map $F \to A$ such that $\pi_0(F) \to \pi_0(A)$ is surjective, the natural map
\begin{equation}
\widehat{\dR}_{A / F} \to \widehat{\dR}_{B / F} \label{eq_goodwillie_dr2}
\end{equation} 
is an isomorphism.

Repeating this trick, we see it suffices to show (\ref{eq_goodwillie_dr2}) is an equivalence if $\pi_0(F) \to \pi_0(A)$ is an isomorphism. Since $\pi_0(F) \to \pi_0(A)$ is an isomorphism, it is surjective, and hence by Corollary \ref{surj_dr_comp} we may identify the map  (\ref{eq_goodwillie_dr}) with 
\begin{equation}\label{eq_comp_must_be_iso}
\Comp(F \to A) \to \Comp(F \to B)
\end{equation}
Since $\pi_0(F) \to \pi_0(A)$ is an isomorphism, we see that $\ker(\pi_0(F) \to \pi_0(B))$ is nilpotent. Hence by Theorem \ref{thm_quillen_convergence_thm_improved} (and Remark \ref{rem_compute_derived_comp}) both sides of (\ref{eq_comp_must_be_iso}) are equivalent to $F$, hence in particular (\ref{eq_comp_must_be_iso}) is an equivalence.
\end{proof}


==> preliminaries.tex <==
\label{sec_notation}
We will use the language of $\infty$-categories as developed in \cite{htt}. By an $n$-category we mean an $\infty$-category in which all mapping spaces are $(n - 1)$-truncated. For example, a $1$-category is an $\infty$-category in which all mapping spaces are discrete. We write $\mathcal{S}$ for the $\infty$-category of spaces, and denote with $\mathcal{S}_{\leq n}$ the full subcategory of $n$-truncated spaces. We write $\Cat_\infty$ for the $\infty$-category of $\infty$-categories. The inclusion 
\[
\mathcal{S} \to \Cat_\infty
\]
has a right adjoint which we will denote by $(-)^\simeq$. 

For an $\infty$-category $\mathcal{C}$, we shall denote with $\sss \mathcal{C}$, resp. $\cc \mathcal{C}$ the $\infty$-category of simplicial, resp. cosimplicial diagrams in $\mathcal{C}$. 

For any stable $\infty$-category $\mathcal{C}$ and $n \in \ZZ$ we shall denote with $[n] \colon \mathcal{C} \to \mathcal{C}$ the $n$-fold composition of the suspension functor \cite[Notation 1.1.2.7]{ha}.

For $k$ a ring, we denote with $\Ch(k)$ the $1$-category of chain complexes over $k$, with $\Ch(k)_{\mathrm{dg}}$ the dg-category of chain complexes over $k$ and with $\derD(k)$ the stable $\infty$-category $\mathrm{N}_{\mathrm{dg}}(\Ch(k)_{\mathrm{dg}})$. Note that we have a canonical functor $\Ch(k) \to \derD(k)$.

If $\mathcal{C}$ is a symmetric monoidal $\infty$-category, we shall denote with $\CAlg(\mathcal{C})$ the $\infty$-category of $\EE_{\infty}$-algebras in $\mathcal{C}$, see \cite{ha}. We will write $\CAlg_k := \CAlg(\derD(k))$, and denote with $\Alg_k$ the $1$-category of discrete commutative $k$-algebras.
\section{Filtrations}
The structure of a partially ordered set on $\NN$ gives $\NN$ the structure of a $1$-category such that there is a unique morphism $i \to j$ if $i \leq j$. We denote $\NN^{\mathrm{disc}}$ for the $1$-category with objects the natural numbers, and all morphisms the identity.
\begin{definition}
Let $\mathcal{C}$ be an arbitrary $\infty$-category. Then we define
\[
\mathcal{C}_\fil := \Fun(\NN^\op, \mathcal{C})
\]
the $\infty$-category of filtered objects in $\mathcal{C}$. For $X \in \mathcal{C}_\fil$, we write $\Fil^i X := X(i)$. Similarly, we let 
\[
\mathcal{C}_\gr := \Fun(\NN^{\mathrm{disc}}, \mathcal{C})
\]
If $\mathcal{C}$ is stable, define a functor $\gr \colon \mathcal{C}_\fil \to \mathcal{C}_\gr$ by 
\[
\gr (X)(i) = \cofib(\Fil^{i + 1}(X) \to \Fil^i(X))
\]
on $X \in \mathcal{C}_\fil$. We will refer to $\gr(X)$ as the \emph{associated graded} of the filtered object $X$, and use the shorthand notation $\gr^i(X) := \gr(X)(i)$. 
\end{definition}

One may give $\NN^{\mathrm{disc}}$ and $\NN^\op$ the structure of a symmetric monoidal category by setting $[p] \otimes [q] := [p + q]$. If $\mathcal{C}$ is symmetric monoidal, the procedure of Day convolution \cite[$\mathsection$2.2.6]{ha} then gives $\mathcal{C}_\gr$ and $\mathcal{C}_\fil$ the structure of a symmetric monoidal category. Explicitly, one has
\begin{align*}
\Fil^n \(X \otimes^\Day Y\) &:= \underset{p + q \geq n}{\colim}\  \Fil^p X \otimes \Fil^q Y \\
(A \otimes^\Day B)(n) &:= \underset{p + q = n}{\bigsqcup}\  A(p) \otimes B(q)
\end{align*}
for $X, Y \in \mathcal{C}_\fil$ and $A, B \in \mathcal{C}_\gr$. Moreover, $\gr$ has a canonical structure of a symmetric monoidal functor, that is there exist canonical isomorphisms
\[
\gr^n \(X \otimes^\Day Y\) \cong \underset{p + q = n}{\bigsqcup}\  \gr^p X \otimes \gr^q Y
\]
for $X, Y \in \mathcal{C}_\fil$. We will denote with 
\begin{equation}\label{proj_i}
\pi^\gr_i \colon \gr^p(X \otimes^\Day Y) \to \gr^{p - i}(X) \otimes \gr^i(Y)
\end{equation}
the projection on the $i$th component.

\begin{definition}[Filtered $\EE_\infty$-algebras]\label{def_filt_alg}
Let $\mathcal{C}$ be a symmetric monoidal $\infty$-category. We define the $\infty$-category of filtered $\EE_\infty$-algebras in $\mathcal{C}$ as 
\[
\CAlg_\fil(\mathcal{C}) := \CAlg((\mathcal{C}_\fil, \otimes^\Day)).
\]
\end{definition}
\begin{lemma}\label{lem_alg_coprod}
The symmetric monoidal structure on $\CAlg_\fil(\mathcal{C})$ is cocartesian, that is the coproduct of algebras is given by the Day convolution product of their underlying objects. In particular $\CAlg_\fil(\mathcal{C})$ admits finite coproducts.
\end{lemma}
\begin{proof}
See \cite[Proposition 3.2.4.7]{ha}.
\end{proof}
We warn the reader that this is a distinctly different category then $\CAlg(\mathcal{C})_\fil$. For $k$ a discrete commutative ring, we will write $\CAlg_\fil(k) := \CAlg_\fil(\derD(k))$. 

For any stable symmetric monoidal $\infty$-category $\mathcal{C}$ and $p \in \NN$, we have a lax symmetric monoidal functor
\[
\gr^{[0, p)} \colon \mathcal{C}_\fil \to \mathcal{C}_\fil
\]
defined by
\begin{equation}
\Fil^i \gr^{[0, p)}(X) := \begin{cases}
\cofib(\Fil^p X \to \Fil^i X) & i \leq p \\
0 & i > p
\end{cases} \label{aae}
\end{equation}
For any $p < q$ we have a natural transformation $\gr^{[0, q)} \to \gr^{[0, p)}$.  Thus if $\mathcal{C}$ admits all limits, we may define the \emph{completion functor}
\begin{align*}
\widehat{(-)} \colon \mathcal{C}_\fil &\to \mathcal{C}_\fil \\ 
X &\mapsto \widehat{X} := \lim_{p \to \infty} \gr^{[0, p)}(X)
\end{align*}
which is also lax symmetric monoidal. Explicitly, one has
\[
\Fil^p \widehat{X} = \lim_{q \to \infty} \cofib(\Fil^p X \to \Fil^q X)
\]
for any $X \in \mathcal{C}_\fil$. We thus get induced functors
\begin{align*}
\gr^{[0, p]} \colon \CAlg_\fil(\mathcal{C}) \to \CAlg_\fil(\mathcal{C}) \\
\widehat{(-)} \colon \CAlg_\fil(\mathcal{C}) \to \CAlg_\fil(\mathcal{C})
\end{align*}
By \cite[Corollary 3.2.2.4]{ha}, we have an equality
\[
\widehat{(-)} = \lim_{p \to \infty} \gr^{[0, p)}
\]
of functors $\CAlg_\fil(\mathcal{C}) \to \CAlg_\fil(\mathcal{C})$. If one sets $\mathcal{C}_{\fil, \comp}$ to be the full subcategory consisting of those $X \in \mathcal{C}_\fil$ such that the natural map $X \to \widehat{X}$ is an equivalence, one may show the functor $\widehat{(-)} \colon \mathcal{C}_\fil \to \mathcal{C}_{\fil, \comp}$ is left adjoint to the inclusion $\mathcal{C}_{\fil, \comp} \to \mathcal{C}_\fil$. For $X, Y \in \mathcal{C}_{\fil, \comp}$ we will denote 
\[
X \widehat{\otimes} Y := \widehat{X \otimes Y}
\]
and similarly for complete $X, Y \in \CAlg_\fil(\mathcal{C})$. 

Finally we will often use without mention that the functor $\gr \colon \mathcal{C}_{\fil, \comp} \to \mathcal{C}_\gr$ is conservative.
\section{Sheaves and stacks}
\label{extend_functors}
For any $\infty$-category $\mathcal{C}$ equipped with a Grothendieck topology $\tau$, and  any $\infty$-category $\mathcal{D}$ in which all limits exist, we shall denote by $\Shv_{\tau}(\mathcal{C}, \mathcal{D})$ the $\infty$-category of $\mathcal{D}$-valued sheaves on $\mathcal{C}$, see \cite[Definition  7.3.3.1]{htt}. More generally, for any $\infty$-topos $\mathcal{X}$ we shall denote by $\Shv_{\mathcal{D}}(\mathcal{X})$ the category of $\mathcal{D}$-valued sheaves on $\mathcal{X}$, i.e. the category of functors $\mathcal{X}^\op \to \mathcal{D}$ that preserve small limits. 
\begin{definition}
We define
\[
\St_k := \Shv_\fppf((\Alg_k)^\op, \mathcal{S})
\]
the $\infty$-category of \emph{higher stacks} over $k$. 
\end{definition}
By \cite[Proposition 6.2.2.7]{htt}, $\St_k$ has the structure of an $\infty$-topos. We warn the reader that these are \emph{underived} stacks, since $\Alg_k$ is the $1$-category of discrete commutative $k$-algebras. Note that inclusion $\Set \to \mathcal{S}$ induces a functor $\Sch_{/ k} \to \St_k$, so in particular we get a fully faithful Yoneda embedding 
\[
\Spec \colon (\Alg_k)^\op \to \St_k
\]
 (essentially because the fppf topology on affine schemes is subcanonical, see \stacksref{03O4}). 
 
For any $\infty$-category $\mathcal{D}$ in which all limits exist, a functor $\mathcal{F} \colon \Alg_k \to \mathcal{D}$ induces (by right Kan extension) a unique functor $\St_k^\op \to \mathcal{D}$ which we shall also denote by $\mathcal{F}$. 
Explicitly, for any $k$-stack $X$ one has
\begin{equation}\label{def_extend}
F(X) := \lim_{\Spec(R) \to X} \mathcal{F}(R)
\end{equation}
and in particular $\mathcal{F}(\Spec(R)) = \mathcal{F}(R)$. Using \cite[Theorem 4.1.3.1]{htt}, one may show that if $X$ is a scheme, the above can be computed as
\begin{equation}\label{def_extend2}
\mathcal{F}(X) = \lim_{\Spec(R) \subseteq X} \mathcal{F}(R)
\end{equation}
where the limit is over all affine opens $\Spec(R)$ in $X$. 

For any $\infty$-category $\mathcal{D}$ admitting all limits, the inclusion
\[
\Shv_{\mathcal{D}}(\St_k) \subseteq \Fun(\St_k^\op, \mathcal{D})
\]
admits a left adjoint $\mathcal{F} \mapsto \mathcal{F}^\dagger$ called \emph{sheafification}. If $\mathcal{F}$ is a sheaf one has $\mathcal{F}^\dagger(X) = \mathcal{F}(X)$ for all $k$-stacks $X$. 

\section{A survey of animation}
If $A$ is a ring and $M$ is an $A$-module, the functor $- \otimes_A M$ is in general not exact. However, it is exact when restricting to the subcategory of free modules. One may introduce the notion of a free resolution $P_\bullet \to N$ of a general $A$-module $N$, and define
\[
N \otimes^\derL_A M := P_\bullet \otimes_A N
\]
to get a better behaved tensor product. For this to make any sense, one needs a category of free resolutions, and it is well known that $\derD(A)_{\geq 0}$ is a good notion for this category. 

In this section we give a quick survey of \emph{animation}, a technique introduced in \cite{cs19} (based on ideas in \cite{quillen-rings} and \cite[\S 5.5.8]{htt}) to give a general way of achieving the above. Given a $1$-category $\mathcal{C}$ generated under colimits by a full subcategory $\mathcal{C}_0$ of nice (compact and projective) objects, we can form the $\infty$-category $\Ani(\mathcal{C})$ freely generated under sifted colimits of these objects. Given a functor $\mathcal{C} \to \mathcal{D}$ which behaves well on $\mathcal{C}_0$, one then obtains a well-behaved functor $\Ani(\mathcal{C}) \to \mathcal{D}$. 

We will give a quick and by no means complete survey, we urge the reader to read \cite[\S 5.5.8]{htt} and \cite{mao} first. Throughout this section, $n$ can be any natural number or the symbol $\infty$.

\begin{definition}[{\cite[\S 5.5.8]{htt}, \cite[Definition A.18]{mao}}]\label{def_compact}
Let $\mathcal{C}$ be a cocomplete category, and $C \in \mathcal{C}$. We say $C$ is \emph{compact} if the functor $\Map_{\mathcal{C}}(C, -) \colon \mathcal{C} \to \mathcal{S}$ commutes with filtered colimits. 

If $\mathcal{C}$ is a cocomplete $n$-category, we say that $C$ is $n$-projective if the functor $\Map_{\mathcal{C}}(C, -) \colon \mathcal{C} \to \Spaces_{\leq n - 1}$ commutes with geometric realizations. If $n = \infty$, we wil say $C$ is projective. 
\end{definition}
Note that although we work with $n$-projective for general $n$, we shall only be interested in the cases $n = 1$ and $n = \infty$.
\begin{definition}[{\cite[Definition A.22]{mao}}]\label{def_gen}
Let $\mathcal{C}$ be an $n$-category and $S \subseteq \mathcal{C}$ a set of objects in $\mathcal{C}$. We say that $S$ is a \emph{set of compact $n$-projective generators} for $\mathcal{C}$ if
\begin{enumerate}
\item $\mathcal{C}$ is cocomplete.
\item Every $X \in S$ is compact $n$-projective.
\item The set $S$ generates $\mathcal{C}$ under small colimits. 
\end{enumerate}
If there exists a set of compact $n$-projective generators of $\mathcal{C}$, we say that $\mathcal{C}$ is \emph{compact $n$-projectively generated}. If $n = \infty$, we say $\mathcal{C}$ is \emph{compact projectively generated}. 
\end{definition}
\begin{definition}
Let $\mathcal{C}$ a $n$-category which admits finite coproducts. We write
\[
\mathcal{P}_n(\mathcal{C}) := \Fun(\mathcal{C}^\op, \mathcal{S}_{\leq n - 1})
\]
and denote  with $\mathcal{P}_{\Sigma,n}(\mathcal{C}) \subseteq \mathcal{P}_n(\mathcal{C})$ the full subcategory consisting of those functors which preserve finite products. 
\end{definition}

\begin{prop}
 Let $\mathcal{C}$ be an $n$-category, and let $S$ be a set of compact $n$-projective generators for $\mathcal{C}$. Let $\mathcal{C}_0$ be the full subcategory on finite coproducts of objects in $S$. Then the Yoneda embedding $P_{\Sigma, n}(\mathcal{C}_0) \to \mathcal{C}$ is an equivalence.
\end{prop}
\begin{proof}
See \cite[Proposition A.29]{mao}.
\end{proof}
\begin{definition}[{\cite[Definition A.32]{mao}}]
Let $\mathcal{C}$ be a compact $n$-projectively generated $n$-category, let $\mathcal{S}$ be a set of compact and $n$-projective generators, and let $\mathcal{C}_0$ be the full subcategory spanned by finite coproducts of objects in $\mathcal{S}$. We define
\[
\Ani(\mathcal{C}) := \mathcal{P}_{\Sigma, \infty}(\mathcal{C}_0)
\]
the \emph{animation} of $\mathcal{C}$. 
\end{definition}

It is good to observe that $\Ani(\mathcal{C})$ is independent of the choice of compact projective generators for $\mathcal{C}$, see \cite[Remark A.33]{mao}. Note that we have a natural Yoneda embedding $\mathcal{C} \to \Ani(\mathcal{C})$ given by $X \mapsto \Map_{\mathcal{C}}(X, -)$. Moreover, by \cite[Remark 5.5.8.26]{htt}, the Yoneda embedding $\mathcal{C} \to \Ani(\mathcal{C})$ admits a left adjoint $\pi_0$. 


\begin{lemma}\label{ani_gen}
Let $\mathcal{C}$ be a compact $n$-projectively generated $n$-category and let $S$ be a set of compact and $n$-projective generators. Then $\Ani(\mathcal{C})$ is compact projectively generated, and $S$ is a set of compact projective generators.
\end{lemma}
\begin{proof}
By definition, for any $X \in S$ the image in $\Ani(\mathcal{C})$ is compact and projective. Since clearly any element in $\Ani(\mathcal{C})$ can be written as a colimit of objects in $S$, the result follows.
\end{proof}
\begin{definition}Let $\mathcal{C}$ and $\mathcal{D}$ be $\infty$-categories. We denote with 
\[
\Fun_\Sigma(\mathcal{C}, \mathcal{D}) \subseteq \Fun(\mathcal{C}, \mathcal{D}) 
\]
the full subcategory of those functors which preserve filtered colimits and geometric realizations. 
\end{definition}
\begin{prop}[{\cite[Proposition 5.5.8.15]{htt}}]\label{left_kan}
Let $\mathcal{C}$ be a cocomplete $n$-category, and let $S \subseteq \mathcal{C}$ be a set of compact $n$-projective generators for $\mathcal{C}$. Let $\mathcal{C}_0 \subseteq \mathcal{C}$ be the full subcategory spanned by finite coproducts of objects in $S$. Let $\mathcal{D}$ be any $\infty$-category which admits filtered colimits and geometric realizations. 

Then the restriction map
\[
\Psi \colon \Fun_{\Sigma} (\mathcal{C}, \mathcal{D}) \to \Fun(\mathcal{C}_0, \mathcal{D})
\]
induces an equivalence of categories.  Moreover, any $g \in \Fun_{\Sigma} (\mathcal{C}, \mathcal{D})$ commutes with all colimits if and only if $\Psi(g)$ commutes with finite coproducts. Finally, for any $f \in \Fun(\mathcal{C}_0, \mathcal{D})$ the inverse image $\Psi^{-1}(f)$ is given by left Kan extension.
\end{prop}


We end by giving two examples of compact projectively generated categories which are essential to the rest of the text.
\begin{example}
Let $k$ be a ring. The set $S = \{k\}$ is a set of compact $1$-projective generators for the category of discrete $k$-modules $\derD(k)^\heart$. The full subcategory spanned by finite coproducts of objects in $S$ is the $1$-category of finite free $k$-modules. Moreover one has $\Ani(\derD(k)^\heart) \cong \derD(k)_{\geq 0}$. 
\end{example}
\begin{example}
For $k$ a ring, we denote with $\Alg_k$ the $1$-category of commutative $k$-algebras. The set $S = \{k[x]\}$ is a set of compact $1$-projective generators, and the full subcategory $\Poly_k \subseteq \Alg_k$ spanned by coproducts of objects in $S$ is the category of finitely generated polynomial $k$-algebras. The $\infty$-category $\CAlg_k^\an := \Ani(\Alg_k)$ is equivalent to the $\infty$-category of simplicial rings. 
\end{example}

\section{Higher algebraic stacks}
We now give an inductive definition of higher algebraic stacks, following Lurie's thesis \cite{thesislurie}.
\begin{definition}
Let $k$ be a ring. A morphism $f \colon X \to Y$ in $\St_k$ is a \emph{relative $0$-stack} if for any $A \in \Alg_k$ and any map $\Spec(A) \to Y$ in $\St_k$, the fiber product $\Spec(A) \times_{Y} X$ is an algebraic space in the sense of \stacksref{025X}. We say that $f$ is smooth if the maps $\Spec(A) \times_{Y} X \to \Spec(A)$ are smooth.

For $n > 0$, a morphism $f \colon X \to Y$ in $\St_k$ is a \emph{relative $n$-stack} if for any $A \in \Alg_k$ and any map $\Spec(A) \to Y$ in $\St_k$, there exists an effective epimorphism $p \colon U \to \Spec(A) \times_Y X$ which is a smooth relative $(n - 1)$-stack, where $U$ is a disjoint union of affine schemes. We will say that a relative $n$-stack $f \colon X \to Y$ is \emph{smooth} if for all $\Spec(A) \to Y$, the cover $U$ can be chosen to be smooth over $\Spec(A)$.

Finally, we define an \emph{algebraic stack} to be a morphism $X \to \Spec(k)$ which is a relative $n$-stack for some $n \in \NN$. 
\end{definition}

We may similarly define open immersions of relative $n$ stacks inductively.
\begin{definition}
A morphism of relative $0$-stacks is an open immersion if it is an open immersion of algebraic spaces. For $n > 0$, we say that a morphism $U \to X$ of relative $n$-stacks is an \emph{open immersion} if there exists a surjective map $T \to X$ which is a relative $(n - 1)$-stack such that $U_T \to X_T$ is an open immersion. In this case, we say $U \subseteq X$ is an \emph{open substack}. 
\end{definition}

For $G$ an affine group scheme (in the classical sense) we can form a simplicial object
\[
\cdots \stack{7} G \times_{\Spec(k)} G \stack{5} G \stack{3} \Spec(k)
\]
in $\sss \St_k$, see \cite[Definition 4.25]{khanstacks}.  We define the \emph{classifying stack} $\mathrm{B}G$ to be the colimit of this diagram in $\St_k$. One may show $\mathrm{B}G$ is an algebraic $1$-stack. By \cite[Theorem 4.28]{khanstacks}, for any $k$-scheme $X$ one may canonically identify the groupoid $\Map_k(X, \mathrm{B}G)$ with the groupoid of $G$-torsors $T \to X$. 

 \section{Module categories on stacks}
Let $k$ be a ring. For any stack $X$ over $k$, we denote with $\derD(X)$ the stable $\infty$-category defined as 
\[
\derD(X) := \lim_{\Spec(A) \subseteq X} \derD(A)
\]
For $A \in \Alg_k$, we say that an object $\mathcal{E} \in \derD(A)$ is \emph{perfect} if it is compact. For a general $X$ in $\St_k$, we say that $\mathcal{E} \in \derD(X)$ is perfect if the pullback $f^*(\mathcal{E})$ is perfect for all $f \colon \Spec(A) \to X$. We denote with $\Perf(X)$ the full subcategory of perfect objects.  We will say that an object $\mathcal{E} \in \derD(X)$ is finite locally free (of rank $n$) if $f^*(\mathcal{E})$ is a finite locally free $A$-module  (of rank $n$)  in homological degree $0$ for all maps $f \colon \Spec(A) \to X$. We will denote with $\Vect(X)$ the full subcategory of finite locally free modules, and with $\Vect_n(X)$ the full subcategory of finite locally free modules of rank $n$. We will write 
\[
\Pic(X) := \Vect_1(X)^\simeq
\]
We refer to elements $\mathcal{E} \in \Vect(X)$ as \emph{vector bundles}, and to elements $\mathcal{L} \in \Pic(X)$ as \emph{line bundles}. We will write $\mathrm{K}_0(\Vect(X))$ for the abelian group generated by the vector bundles on $X$ with relations coming from short exact sequences, see \stacksref{0FDE}. For $\iota \colon Z \hookrightarrow X$ a closed immersion of schemes and $\mathcal{E} \in \derD(X)$, we will sometimes write $\mathcal{E} \rvert_Z := \iota^*(\mathcal{E})$. 
\begin{lemma}\label{vect_sheaf2}
Let $k$ be a ring. Let 
\[
\mathcal{F} \colon \St_k^\op \to \Cat_\infty
\]
be an element of $\{\derD(-), \Perf(-), \Vect(-), \Vect_n(-), \Pic\}$. Then $\mathcal{F}$ is a sheaf (for the fppf topology).
\end{lemma}
\begin{proof}
For $\derD(-)$ this follows from \cite[Corollary D.6.3.3]{sag}. Since the condition that an object is perfect or locally free (of rank $n$) is local for the flat topology by \cite[Proposition 2.8.4.2]{sag}, the rest follow by \cite[Corollary 3.3.3.2]{htt}.
\end{proof}

